A Universal Machine for Biform Theory Graphs

Broadly speaking, there are two kinds of semantics-aware assistant systems for mathematics: proof assistants express the semantic in logic and emphasize deduction, and computer algebra systems express the semantics in programming languages and emphasize computation. Combining the complementary strengths of both approaches while mending their complementary weaknesses has been an important goal of the mechanized mathematics community for some time. We pick up on the idea of biform theories and interpret it in the MMTt/OMDoc framework which introduced the foundations-as-theories approach, and can thus represent both logics and programming languages as theories. This yields a formal, modular framework of biform theory graphs which mixes specifications and implementations sharing the module system and typing information. We present automated knowledge management work flows that interface to existing specification/programming tools and enable an OpenMath Machine, that operationalizes biform theories, evaluating expressions by exhaustively applying the implementations of the respective operators. We evaluate the new biform framework by adding implementations to the OpenMath standard content dictionaries.

==> impl.tex <==
\svnInfo $Id: impl.tex 1131 2013-03-01 07:33:41Z kohlhase $
\svnKeyword $HeadURL: https://svn.kwarc.info/repos/frabe/Papers/omdoc-spec/openmath/uom/impl.tex $

%% FR: we should discuss related work here, but better nothing than mention only one system
% The Kenzo system~\cite{kenzo} is a computer program devoted to symbolic computation in
% Algebraic Topology. In~\cite{kenzo_med_access} and~\cite{omdoc_computer_algebra}, the
% authors present an architecture to dynamaically load new modules in a Graphical User
% Interface (GUI) for the Kenzo system by encoding information on the user interface
% specification and the code carrying the functionality of the GUI in the \omdoc and
% \openmath formats. The authors are embedding pieces of program code into \omdoc documents
% by using the \lstinline|<code>| tag and then dynamically create GUIs for specific
% documents using the code.


%   \section{Preliminaries}
%   In this section we present a very brief overview of the \openmath and \omdoc standards.
% 
%   \subsection{\openmath}
%   \openmath~\cite{openmath} is a standard for representing mathematical data in as
% unambiguous a way as possible. It can be used to exchange mathematical objects
% between software packages or via email, or as a persistent data format in a
% database. It is tightly focussed on representing semantic information. Formally,
% an \openmath object is a labelled tree whose leaves are the basic \openmath
% objects integers, IEEE double precision floats, unicode strings, byte arrays,
% variables or symbols. \openmath objects can be built up recursively in a number
% of ways. One of them is function application, another is attribution, which can
% be used to add additional information to an object without altering its
% foundational meaning. Another example is binding objects which are used to
% represent an expression containing bound variables. 
% 
%   \subsection{\omdoc}
%   Open Mathematical Documents (\omdoc)~\cite{omdoc} is an open markup language for
% mathematical documents. It is designed to provide a semantics-oriented
% infrastructure for the communication and storage of mathematical knowledge. The
% representation in \omdoc makes the document content unambiguous and its context
% transparent. \omdoc achieves this by employing document markup, specifically by
% embedding control codes into mathematical documents that identify the structure
% of the document, the meaning of text fragments, and their relation to other
% mathematical knowledge. The main design principles behind the \omdoc format are
% for it to be ontologically uncomitted, to combine formal and informal views of
% the mathematical knowledge in its documents, to be based on sound logic and
% representational principles and to be based on structural content markup. In
% addition, \omdoc documents have the capability to provide for semantic markup and
% therefore allow for documents that are benefitting from this to be mechanically
% processed by proof verification software, thereby certifying the corectness of
% the proofs. Thus, the \omdoc format provides representations that can easily be
% read by humans and representations that allow for an advanced level of machine
% support.

%   \section{Description of the System}
%   In this section we describe the Universal \openmath Machine by first
% introducing the reader with a general overview and then providing a more
% detailed explanation of the inner workings of the system.

In this section we will provide a general description of the Universal \openmath
Machine. Source code and deployment instructions can be found in our \mmt SVN
repository~\cite{project:mmt}.

The Universal \openmath Machine is designed to evaluate or simplify \openmath expressions
which are composed of \openmath objects that are part of \omdoc documents and for which
there exist written Scala algorithmic implementations that define how an \openmath
expression can be simplified into another \openmath object. The UOM is deployed as a web
service which users can easily access via a web browser or any other program that can send
an HTTP~\cite{httprfc} request. Users interact with the system in a straightforward manner
by just passing an \openmath object to it. Also, users can upload documents or even
precompiled implementations to the system. Authors of documents or implementations have to
follow a small set of simple rules to make their work exploitable by the UOM. The UOM
consists of several components that interact together. The major steps that need to be
performed by the UOM in order to respond to a request by a client are to recursively
simplify an expression by searching for \openmath objects with implementations, parsing
relevant \omdoc documents and generating Scala source files from them, compiling the scala
code and maintaining an implementation database cache and finally executing
implementations when needed in order to simplify or evaluate \openmath objects.
% The inner workings of the UOM are
% described in greater detail in subsection \ref{sec:implem_details}.

\subsection{The UOM web service}

The UOM provides a web service that can be accessed by any user who is
running a web browser on his computer. This makes the service available to
a very wide spectrum of devices. Users of the service can also benefit from the client-server model in
several ways. 

One of them is that users are not required to have a Scala
compiler or interpreter installed, which makes the service accessible also to
users that cannot program in Scala or any language at all, and it also reduces
the computational load on the user's computer. The UOM service can be deployed
on powerful servers which can in turn reduce the time needed to produce a
response to the request compared to the time it would take should the service
be running locally on the user's computer. Moreover, the UOM server can
dynamically keep an implementation database cache, a database where
implementations of \openmath objects are precompiled and ready to use, which
would produce faster response times and makes the client-server model even more
beneficial.

Another advantage of the client-server model is that users will not be
required to deploy any additional software on their machines and will not be
bothered with any support, maintenance or system administrative tasks involved
with running the software. In addition, users will be safe from any security or
privacy vulnerabilities that might arise from executing malicious third-party
code embedded in an \omdoc document. Clearly, optimising performance and coping
with potential security issues requires a degree of knowledge or effort which
some users do not have or are unwilling to make, which is another reason to
employ the client-server model.

\subsection{User interaction}

All that is required from the user in order to utilize the UOM is to send an
HTTP request which encodes an \openmath object. Every atomic
subterm of the object refers to an \omdoc constant or other element that has
a unique URI~\cite{URI}, associated with it. This is all of the information
required by the UOM in order to produce a response. In the current version of
the system, the user would have to upload documents or implementations to the
system if there are \openmath terms whose URIs refer to documents that are not
on the server, however in future versions of the service, support for
automatically retrieving documents based on the URIs of the \openmath objects
can be implemented. 

A universal way to access
the UOM from any device would be to use an online web interface that provides
the necessary features. Such a feature could be browsing through a catalogue of
\omdoc documents and having the ability to select theories or constants within
it. Another would be to have a tool that allows constructing user objects from
already existing \openmath objects in other documents.

Once the request has been made on behalf of the user the response time depends
on several factors. Excluding external factors to the software (e.g. server
load, network latency, etc.), there are two main performance bottlenecks of the
system. The first one is the compilation step which can be avoided if the
required implementations are already registered in the database. That would be
the case for recently accessed documents or for documents that are popular
among the users. The second performance hurdle could potentially come from the
execution of the implementation. Poorly written implementations or
implementations of functions that are inherently complex might take considerable
time to execute. However, there would be many use cases where the response time
would be comparable to that of a website. One such use case would be responding
to a request for which all of the implementations are in the database (for
instance the document is stored on the same machine as the UOM) and the
complexity of the implementations is negligable.

\subsection{Document Requirements}

Special requirements when creating an \omdoc document apply only to constants that are to
have Scala implementations written for them. Implementations are allowed only for elements
at the object level that are represented as \openmath objects. The Scala implementations
should be enclosed in \lstinline|<OMFOREIGN>| tags. The implementation for a single
\openmath object does not have to be self-contained in the sense that it can be compiled by
the Scala compiler on its own. The implementation can implicitly rely on other \openmath
objects which are referenced in the same or different \omdoc documents. Each implementation
should use the \mmt API~\cite{project:mmt} data structure which represents \openmath objects
- \lstinline|Term| - in the sense that all of the input parameters are \lstinline|Term|
and also the return value of the implementation is \lstinline|Term| as well.

Authors should know that \omdoc theories are translated to Scala classes. The
full binary name of the class is formed from the URI of the theory which removes
the possibility for naming conflicts. Constants from theories are translated
to member fields of the corresponding class. This provides a convenient way for
users to refer to any \omdoc constant when writing implementations. In
addition, authors should use theory inclusions when their implementations are
referencing \openmath objects from different documents or theories.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.5]{diagram.jpg}
    \caption{System framework} 
    \label{fig:framework}
\end{figure}

%   \subsection{Implementation Details}\label{sec:implem_details}
%   In this section we describe the important computational steps that the UOM
% performs in order to evaluate the request of the user and also describe the
% different components of the system. The system has three main components -  the
% extractor, the implementation database and the main controller.
% 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.5]{diagram.jpg}
%     \caption{System framework} 
%     \label{fig:framework}
% \end{figure}
% 
%   \subsubsection{Extractor}
%   The extractor is the component of the system whose task is to generate Scala
% files from \omdoc documents. Given an \omdoc document, the extractor parses it
% and translates the different theories found in the document to Scala
% classes. In order to avoid naming conflicts, the extractor creates unique
% binary names for every class that corresponds to an \omdoc theory. Each class is
% written as part of a package, whose name is derived from the URI of the
% document in the traditional way. Therefore, all \omdoc theories in a single
% document will be translated to classes with the same package name. The name of
% the class inside the package is then just the name of the corresponding \omdoc
% theory. 
% 
% Given an \omdoc theory, the extractor will translate the \omdoc constants
% that do not have an implementation to member value fields of the class
% with the same name as the constants. Constants with implementation are
% written to the Scala source file as methods. The implementation is taken
% verbatim from the document and the author should write it exactly as it would
% appear in a Scala class, including the \textbf{def} keyword, signature, return
% type, etc. This allows for implementations that take variable number of
% \openmath terms as input parameters. In addition, the extractor generates
% an auxiliary method and member field value in order to provide a
% universal way of accessing implementations from the main controller
% using reflection. 
% 
% Lastly, the extractor also handles theory inclusions by first
% checking if the theory to be included has been translated. If it is not, then
% the extractor retrieves it and translates it.
% 
%   \subsubsection{Implementation Database}
%   The implementation database is used by the UOM to store precompiled
% implementations that are associated with an \openmath object. The benefit that
% the implementation database brings to the UOM is faster response times for
% implementations that are stored by avoiding the compilation, which is otherwise
% necessary and computationally expensive. Currently, the database is stored
% entirely in main memory and is simply a Scala HashMap that associates the unique
% names of \openmath objects to implementations. In future versions of the
% system, the database can be improved by making it persistent and storing it on
% the file system, but for our current purposes, it is enough to store it in
% memory as a proof-of-concept. Updating the database is done by providing a
% jar
% file which contains a collection of class files. The UOM uses Java reflection
% on the class files and stores the implementations into the HashMap making them
% ready to use on demand.
% 
%   \subsubsection{Main Controller}
% 	The main controller performs several functions. It interacts with the
% operating system in order to provide some of the needed functionality (e.g. 
% call the scala compiler, the jar utility etc.). It also controls the general
% flow of the program by invoking methods in the other components. The main 
% controller also receives the request of the client and identifies subterms,
% within the \openmath term to be evaluated, for which implementations need to
% be obtained. The main controller first consults the database to check if 
% there are any implementations that are already available. For the rest, 
% if any, the controller will, in future versions of the system, retrieve the
% documents that are required and pass 
% them to the extractor. In the current version, the user is required to
% upload his document or precompiled implementation to the server if the
% implementation or document are not stored there. Once the extractor has
% completed its work, the main
% controller compiles the scala Source files using the Scala compiler, and 
% creates a jar file from the collection. The jar file is then passed to the
% implementation database and all the extracted implementations are registered
% with it. Finally, a response can be produced to the client, by recursively
% simplifying the term in the request using the implementations in the 
% database. The interactions are illustrated in figure \ref{fig:framework}.


We describe an application scenario where the Universal \openmath Machine can be used for
web-based education and we also illustrate the different computational steps by using an
example \omdoc document.
%In \ref{sec:unit} we present a use case
%for the UOM in unit conversion.

The system allows a user to view \omdoc documents
and evaluate expressions of interest using a web browser on a low-end computer
that has very limited software installed, in particular lacking the capability
of executing Scala code. The system is designed to perform the computationally
intensive tasks on the server, so the client is not required to run on a
powerful computer. Students and other readers learning about mathematical
theories can benefit from the system as it will provide a more interactive
learning experience by allowing students to evaluate and simplify relevant
mathematical objects from those theories. The reader will also be able to
evaluate examples that were created by himself. 

First, we present a standard \omdoc document without any implementations embedded 
into it and briefly describe it. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Document without implementations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
\small
\begin{verbatim}
<omdoc xmlns="http://omdoc.org/ns" base="http://cds.omdoc.org/unsorted/uom.omdoc">
   <theory name="lists">
     <constant name="elem"/>
     <constant name="list"/>
     <constant name="nil"/>
     <constant name="cons"/>
     <constant name="append"/>
   </theory>

   <theory name="lists_ext">
     <include from="?lists"/>
     <constant name="append_many"/>
   </theory>
</omdoc>
\end{verbatim}

\normalsize

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Document with implementations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The theory \textit{lists} introduces the basic components needed to represent
the list data structure which can be found in LISP and many functional
programming languages. In addition, using the basic objects \textit{elem, list,
nil, cons}, we can define the function \textit{append} which given two lists
returns the list formed by appending the second one to the first list. The
second theory - \textit{lists\_ext} - extends the first theory by 
introducing a new fucntion called \textit{append\_many}. Given any number of 
lists as parameters, the function should return the list formed by appending all 
of the lists consecutively given the order. 

Using the above document as a base, implementations can easiliy be added. Every constant
that requires an implementation should be given a definition as an \lstinline|OMFOREIGN|
object according to the \omdoc standard. The document with embedded definitions is
displayed below with the Scala implementations colored in blue.

\small
\begin{verbatim}
<omdoc xmlns="http://omdoc.org/ns" base="http://cds.omdoc.org/unsorted/uom.omdoc">
   <theory name="lists">
     <constant name="elem"/>
     <constant name="list"/>
     <constant name="nil"/>
     <constant name="cons"/>
     <constant name="append">
       <definition>
         <OMOBJ>
           <OMFOREIGN>
\end{verbatim}
{
\color{blue}
\begin{verbatim}
             def append(l: Term, m: Term) : Term = {
               l match {
                 case this.nil => m;
                 case OMA(this.cons, List(this.elem, rest)) => 
                    OMA(this.cons, List(this.elem,  append(rest, m)) );
                 case _ => throw new Exception("malformed term");
               }
             }
\end{verbatim} 
} 
\begin{verbatim}
           </OMFOREIGN>
         </OMOBJ>
       </definition>
     </constant>
   </theory>

   <theory name="lists_ext">
     <include from="?lists"/>
     <constant name="append_many">
       <definition>
         <OMOBJ>
           <OMFOREIGN>
\end{verbatim}
{
\color{blue}
\begin{verbatim}
             def append_many(l: Term*) : Term = {
               val lists = new org.omdoc.cds.unsorted.uom.omdoc.lists;
               l.toList match {
                 case Nil => lists.nil
                 case hd :: tl => lists.append(hd, append_many(tl : _*))
               }
             }
\end{verbatim}
}
\begin{verbatim}
           </OMFOREIGN>
         </OMOBJ>
       </definition>
     </constant>
   </theory>
</omdoc>
\end{verbatim}

\normalsize

For this scenario, we have selected a short document which nonetheless captures the
essential problems that the system will have to overcome, namely implementations
using other implementations of \openmath objects defined in different theories.  
The implementation written for \textit{append\_many} relies on
\textit{append} and uses the objects from the first theory - \textit{lists}.

Suppose the user would like to evaluate the expression from the above theory
which represents the list  
  \textbf{\textit{append\_many}([1,2,3], [4,5], [6,7])}       
  The browser sends a request to the UOM server specifying the expression of
interest. The UOM first consults the implementation database and then, it
identifies the \omdoc
document which is reffered by the \openmath objects and the system generates
a Scala source file. Once the source file has been created, the UOM compiles it, produces a jar
file which is used by the implementation database to register the
implementations for the \openmath objects that need to be evaluated. Then, the
UOM simplifies the expression using the implementations and the result of the
execution is the \openmath expression which is equivalent to the list
\textbf{[1,2,3,4,5,6,7]}. The result is then sent back to the client and the
browser can render it on the screen.  

%   \subsection{Unit Conversion}\label{sec:unit}
%   In~\cite{mcirlanaru:bscthesis}, the author proposes a framework for
% unit conversion in technical documents. The framework encompasses many
% different systems, technologies and formats in order to enable interactive
% unit conversion to the reader. As part of the framework, the author uses the
% UOM web service for the arithmetic computations that are required in order to
% present correct unit conversions to the reader. In the stage where the UOM is
% used, the Universal \openmath Machine receives an \omdoc document containing
% unit quantities that need to be simplified or evaluated arithmetically. For
% that purpose, the UOM is preloaded with the implementations of the
% \openmath symbols used to denote the common arithmetic operations of addition,
% subtraction, division and multiplication which are used throughout the
% framework. After performing the arithmetic evaluations, the UOM web
% service returns the simplified \omdoc document, which is used by the framework
% to eventually produce Presentation MathMl~\cite{mathml} + \openmath.

%%% Local Variables: 
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End: 


==> pgflibrarytikzmmt.code.tex <==
\usetikzlibrary{arrows}
\newcommand{\mmtarrowtip}{angle 45}
\newcommand{\mmtarrowtipepi}{triangle 45}
\newcommand{\mmtarrowtipmono}{right hook}
\tikzstyle{thy}=[draw,outer sep=1mm,rounded corners]
\tikzstyle{include}=[\mmtarrowtipmono-\mmtarrowtip,thick]
\tikzstyle{view}=[dashed,-\mmtarrowtip,thick]
\tikzstyle{struct}=[-\mmtarrowtip,thick]
\tikzstyle{meta}=[dotted,-\mmtarrowtip,thick]
\tikzstyle{morph}=[-\mmtarrowtip] % any morphism
\tikzstyle{mapsto}=[|-\mmtarrowtip] % any morphism



==> tikzlibrarymmt.code.tex <==
\input{pgflibrarytikzmmt.code.tex}

